Design and Implementation of the Cosmic Ray Tagger System for the ICARUS detector at FNAL

The ICARUS-T600 Liquid Argon Time Projection Chamber is operating at Fermilab at shallow depth and thus exposed to a high flux of cosmic rays that can fake neutrino interactions. A cosmic ray tagging (CRT) system ($\sim$1100 m$^2$), surrounding the cryostat with two layers of fiber embedded plastic scintillators, was developed to mitigate the cosmic ray induced background. Using nanosecond-level timing information, the CRT can distinguish incoming cosmic rays from outgoing particles from neutrino interactions in the TPC. In this paper an overview of the CRT system, its installation and commissioning at Fermilab, and its performance are discussed.

==> top_side_febs.tex <==
The front-end boards (FEBs) for the Top and Side CRT systems were designed by Igro Kreslo and others at the University of Bern specifically for the MicroBooNE and SBND CRT designs, providing the minimum cost per electronics channel. A full discussion of the requirements and the functionality of the Bern FEB design can be found in \cite{feb}. For convenience, we reproduce a summary below. The FEB
\begin{enumerate}
\item provides bias voltage in the range of 20-90~V individually adjustable for each of 32~SiPMs;
\item amplifies and shapes the SiPM output pulse on each of 32~channels (Fig.~\ref{fig:feb_analog});
\item performs discrimination of shaped signals at configurable level equivalent to 0 to 50 photoelectrons (PEs);
\item allows for requiring coincidence of signals from each pair of adjacent channels (optional); 
\item allows for triggering only on events that are validated by external signals, such as by a signal in a group of other FEBs (Fig.~\ref{fig:feb_trig}); 
\item generates a trigger for digitization of all 32 signal amplitudes; 
\item generates a time stamp with respect to the input reference pulse with an accuracy of 1.3~ns~RMS; 
\item  performs digitization of the signal amplitude of each of the 32 channels; 
\item  provides on-board data buffering; 
\item  provides efficient back-end communication based on the 100~Mbps Ethernet standard; 
\item  allows firmware upgrade via back end Ethernet link;
\item  requires input power 5~V with the consumption ranging from 450~mA to 550~mA depending on channel configuration.
\end{enumerate}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.9\linewidth]{ImagesSide/feb.pdf}
    \caption{The CAEN A1702/DT5550 32-channel front-end board~\cite{feb} is used for all SBN CRTs.}
    \label{fig:feb}
\end{figure}
The FEB was originally designed to readout a single CRT module consisting of 16 scintillator strips, each with two WLS fibers. SiPMs are known to be noisy devices with typical dark rates in the range of kHz–MHz. To reduce the rate of false triggers due to dark noise, an approximate 30-ns coincidence gate is applied to channels x and x+1 with x = 0,2,4,...,30. This coincidence window is optimized for the SBND geometry. Furthermore, the FEB can be configured to require an external validation signal in order to trigger a readout. See Figure~\ref{fig:feb_trig}.  The intended use of this feature is to generate coincidence gates between FEBs reading out scintillator modules in adjacent layers. The SBND CRT has two layers of modules, where each module is read out by a single FEB. The two layers are arranged perpendicular to each other in a X-Y layout, providing the approximate point of entry of a cosmogenic muon. When any of the single strips in a layer generates a signal above threshold, a validation pulse is sent out from that FEB to the FEBs in the adjacent layer. The event is validated if coincidence across two layers is observed within 150~ns, the maximum delay incurred for a validation signal due to SBND's cable layout. If a readout occurs, the triggered FEBs incur a 22-$\mu$s deadtime. Otherwise, the deadtime is reduced to the coincidence gate width of 150~ns.

\begin{figure}[h]
    \centering
    \begin{subfigure}{\textwidth}
    \centering
    \includegraphics[width=0.85\linewidth]{ImagesSide/feb-analog-processing.pdf}
    \subcaption{FEB analog readout circuit.}
    \label{fig:feb_analog}
    \end{subfigure}
    \begin{subfigure}{\textwidth}
    \centering
    \includegraphics[width=0.85\linewidth]{ImagesSide/feb-trigger-circuit.pdf}
    \subcaption{FEB trigger circuit.}
    \label{fig:feb_trig}
    \end{subfigure}
    \caption{The FEB provides full analog readout and digitization (a) with configurable trigger logic (b) as shown in the block diagrams~\cite{feb}. }
    \label{fig:feb_block_diagrams}
\end{figure}

Individual FEBs can be daisychained through the Ethernet interface, up to 256 in total, on a single network for easy interfacing with a single PC. Slow control of the FEB via the Ethernet interface facilitates real-time configuration of the preamplifier gain, SiPM bias voltage, and discriminator threshold values. For small-scale applications, this functionality is provided through a standalone DAQ software package equipped with a dedicated GUI. The software is written in a combination of C and ROOT6, and data is written in root tree format for quick analysis. In addition, the software provides real-time, low-level analysis results including charge spectra for each FEB channel, trigger rate, and period measurements for the timing signals.
